Separability in the Ambient Logic

The \it{Ambient Logic} (AL) has been proposed for expressing properties of process mobility in the calculus of Mobile Ambients (MA), and as a basis for query languages on semistructured data. We study some basic questions concerning the discriminating power of AL, focusing on the equivalence on processes induced by the logic $(=_L>)$. As underlying calculi besides MA we consider a subcalculus in which an image-finiteness condition holds and that we prove to be Turing complete. Synchronous variants of these calculi are studied as well. In these calculi, we provide two operational characterisations of $_=L$: a coinductive one (as a form of bisimilarity) and an inductive one (based on structual properties of processes). After showing $_=L$ to be stricly finer than barbed congruence, we establish axiomatisations of $_=L$ on the subcalculus of MA (both the asynchronous and the synchronous version), enabling us to relate $_=L$ to structural congruence. We also present some (un)decidability results that are related to the above separation properties for AL: the undecidability of $_=L$ on MA and its decidability on the subcalculus.

==> tableRED.tex <==
\begin{table*}[ht]
$$\begin{array}{cc}
\multicolumn{2}{c}{
 \shortaxiomC{ \openamb n . P |
\amb n{ Q} \longrightarrow 
P |  Q
}
{Red-Open} 
}
\\[\tkpP]
\multicolumn{2}{c}{
  \shortaxiomC
{ \amb n {\inamb m . P_1 | P_2} | 
\amb m{ Q} \longrightarrow 
\amb m{ \amb n { P_1 | P_2}| Q
}}{Red-In}
}
 \\[\tkpP]
\multicolumn{2}{c}{ 
 \shortaxiomC
{
\amb m{ \amb n {\outamb m . P_1 | P_2}| Q}
\longrightarrow 
 \amb n {P_1 | P_2} | 
\amb m{ Q} 
}
{Red-Out}  
}
 \\[\tkpP]
\multicolumn{2}{c}{ 
 \shortaxiomC
{ \msg n |
\abs m  P \longrightarrow 
P \sub n m
} 
{Red-Com}
}
\\[\tkpP]
\shortinfruleN
{
 P  \longrightarrow  P'
}
{
P |Q  \longrightarrow  P' |Q
}
{Red-Par}
&
\shortinfruleN
{
 P   \longrightarrow  P'
}
{
\amb n P   \longrightarrow  \amb n {P'}
}
{Red-Amb}    %\qquad
 \\[\tkpP]
\multicolumn{2}{c}{ 
\shortinfruleN
{
 P \equiv P' \andalso P'  \longrightarrow  P'' \andalso P'' \equiv P'''
}
{
P   \longrightarrow  P'''
}
{Red-Struct}
}\end{array} 
$$%\]
\caption{The rules for reduction}
\Mybar  
\label{t:red_rules}
\end{table*}


==> tableSYN.tex <==

\begin{table*}[ht]
\begin{center}
\begin{tabular}{cc}
$
\begin{array}[t]{lrll}
%\\[\tkp]
\multicolumn{3}{l}{ 
a,b, \ldots, n,m } & {\mbox{\it Names}}
%  \multicolumn{3}{l}{
%   h,k, \ldots n,m}
%& {\mbox{{\it Names}}} %\\[12pt]
%\\[\tkp]
%  \multicolumn{3}{l}{
%   \eta}
%& {\mbox{{\it Names $\cup$ Variables}}} 
\\[6pt]%[\tkp]
 &&& {\mbox{\it Capabilities}}
\\[\tkp] 
\capa & ::=
   &  \inamb n 
   & \mboxB{enter}
\\[\tkp]
 & \midd
   &  \outamb n %  \eta
   & \mboxB{exit}
\\[\tkp]
 & \midd
   &  \openamb n %  \eta
   & \mboxB{open}
\end{array}
$ \qquad \qquad \qquad& 
$\begin{array}[t]{lrll}
 &&& {\mbox{\it Processes}}
\\[\tkp] 
P,Q,R & ::=  
   & \nil
   &
   \mboxB{nil}
\\[\tkp]
 & \midd
   & P |  Q
   & \mboxB{parallel}
\\[\tkp]
 & \midd
   & \capa . P
   & \mboxB{prefixing}
\\[\tkp]
 & \midd
   & (n)\,P
   & \mboxB{abstraction}
\\[\tkp]
 & \midd
   & \msg n
   & \mboxB{message}
\\[\tkp]
 & \midd
   & n[P]
   & \mboxB{ambient}
   \\[\tkp]
   & \midd
   & !P
   & \mboxB{replication}
\end{array} 
$
\end{tabular}
\end{center} 
 \caption{The syntax of public \MA}
\Mybar  
\label{ta:syn}
\end{table*} 

